Visually grounded few-shot word learning in low-resource settings

We propose a visually grounded speech model that learns new words and their visual depictions from just a few word-image example pairs. Given a set of test images and a spoken query, we ask the model which image depicts the query word. Previous work has simplified this few-shot learning problem by either using an artificial setting with digit word-image pairs or by using a large number of examples per class. Moreover, all previous studies were performed using English speech-image data. We propose an approach that can work on natural word-image pairs but with less examples, i.e. fewer shots, and then illustrate how this approach can be applied for multimodal few-shot learning in a real low-resource language, Yor\`ub\'a. Our approach involves using the given word-image example pairs to mine new unsupervised word-image training pairs from large collections of unlabelled speech and images. Additionally, we use a word-to-image attention mechanism to determine word-image similarity. With this new model, we achieve better performance with fewer shots than previous approaches on an existing English benchmark. Many of the model's mistakes are due to confusion between visual concepts co-occurring in similar contexts. The experiments on Yor\`ub\'a show the benefit of transferring knowledge from a multimodal model trained on a larger set of English speech-image data.

==> analysis.tex <==
\newpage~\newpage~\newpage~\newpage~\newpage~\newpage
\section{Further Analysis}

\begin{itemize}
    \item Start off with essence of our approach: pair mining.
\end{itemize}

\subsection{The contribution of the mined pairs}

\begin{itemize}
    \item To determine the mined pairs' contribution to this performance boost, we do an experiment where we do not update \model\ on the mined pairs after pretraining it on the background data (not containing any of the few-shot classes). 
    To test this model on the few-shot retrieval task, we use the indirect few-shot method of \cite{eloff_multimodal_2019, nortje_unsupervised_2020}: each $\boldsymbol{\mathrm{x}}^q_{\textrm{audio}}$ is compared to each $\boldsymbol{\mathrm{x}}_{\textrm{audio}}^{(j)}$ in $\mathcal{S}$ to find the audio example closest to the query.
    The image $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^{(j)}$ corresponding to the closest $\boldsymbol{\mathrm{x}}_{\textrm{audio}}^{(j)}$ is then used to calculate the similarity to each image $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^{(i)}$ in $\mathcal{M}$.
    Using mined pairs improves the scores with roughly 20\% when comparing lines~1 and 2.

\item For the no pair mining method, the scores are worse and drops slightly as $K$ increases. When looking at the few-shot task, we see the mined pairs contributes even more to the few-shot task, even though it only has to distinguish between 5 images instead of 5000 (as for retrieval).

\item However, this simply proves that it is crucial for the model to be updated with the few-shot classes. What if the model is only updated on the ground truth samples from the support set?
\item For higher shots, $K >= 50$, the naive approach produces higher scores. But for lower shots, $K < 50$, the few-shot scores are lower for the naive approach.

\item Similarly, with increasing K, the few-shot retrieval scores gets to the overall score when using mined pairs. Thus, for fewer shots we can get to (or close to) the few-shot and retrieval scores for large values of K for the naive approach.

\item Without the mined pairs and base negatives, we thus do not see the plateau in retrieval scores. It seems that with enough training pairs, we can reach that plateau faster. But what in the mined pairs causes this plateau in retrieval scores but not few-shot scores?
\end{itemize}

\subsection{Per keyword performance}
\label{subsec:per_keyword_performance}

Table~\ref{tab:keyword_analysis} presents the retrieval performance for each of the five keywords considered.
We observe a large variance in performance across the concepts:
``fire hydrant'' is the most challenging keyword to retrieve (with a performance as low as 0\% $P$@N),
while ``zebra'' is the easiest (reaching a precision of over 83\%).
Figure~\ref{fig:per_keyword_40_classes}, which shows the scores for forty concepts,
confirms the wide range of performances.
The differences between keywords could be due to a number of factors,
object size and word frequency being probably among the most important ones, as suggested by Miller and Harwath \cite{miller_t_exploring_2022} in a related study (Table 4 in their paper).

Interestingly, if we look at how the performance varies with the number of shots $K$,
we get a more nuanced picture than the one provided by the aggregated results (Table~\ref{tab:previous_work}).
While we previously observed the aggregated performance staying approximately constant with $K$,
here we instead see that there are variations in both directions depending on the keyword:
the retrieval scores improve with $K$ for ``sheep'', but degrade for ``fire hydrant'' and ``kite.''
We speculate that as $K$ increases, the model becomes more dependent on the recurring contextual (background) features, which are especially difficult to disentangle for the objects that occupy only a small part of the image (``fire hydrant'', ``kite'');
see Figure~\ref{tab:qualitative-results} for some examples of the top ranked images together with their visual explanations.

\subsection{The retrieval score plateau}
\label{subsec:retrieval_plateau}

    
\begin{itemize}
    \item Why does the few-shot classification scores (Table~\ref{tab:few-shot}) increase for \model\ (with sampling), but the few-shot retrieval (Table~\ref{tab:previous_work}) scores stay relatively the same?
    \item The scores of the audio and image pairs increase as $K$ increases -- although increase is not that much.
    
    \item Maybe its the task and not the model? I.e.\ the task is equally difficult and the improvement of pairs does not influence the model's ability to do the task?
    \item However, looking at the per keyword retrieval scores in Table~\ref{tab:keyword_analysis} we see that performance for some keywords stay relatively the same (\textit{broccoli} and \textit{zebra}), while others improve (\textit{sheep}) and others decline (\textit{fire hydrant} and \textit{kite}). As a result the scores almost evens out.
    
    \item But why does this actually happen? In Table~\ref{tab:retrieval-vs-classification}, we show that for these classes, the model depends on the contextual information to identify the class. In the classification task, this doesn't have such a significant effect since the few-shot classes and their contexts are quite distinct from one another. But when it comes to retrieval, we see that the model focusses more on the contextual data than the actual visual concept.
    
\end{itemize}


\subsection{Increasing the number of classes}
\label{subsec:testing_L}




\begin{itemize}
    \item To further analyse what happens with more classes... 
    \item The retaining of contextual information should also become evident if we increase the amount of few-shot classes: the more classes, the more difficult it is to distinguish between the few-shot images in the matching set. 
    \item In the final line of Table~\ref{tab:mining_vs_no_mining_retrieval} we start to investigate how our approach performs when, instead of using just five few-shot classes, we have 40 few-shot classes to learn with $K = 5$ shots. We see that we pay roughly 5\% in $P@N$, but even when learning 40 classes, we still outperform the five-class oracle masking approach across all shots considered.
    \item Looking at the five-shot case, we see that training on more classes ($L_{\mathcal{S}}=40$) leads to a slightly lower classification score on the original five classes.
The few-shot accuracy when tested on all 40 classes is 21.7\%. %

\end{itemize}

\subsection{The effect of the base image negatives}
\label{subsec:base_images}


\begin{itemize}
    \item Ideally, the usage of base negative images should force the model to throw away more contextual information, but does it? It does lower the overall retrieval scores, which makes sense since the model is not forced to distinguish the few-shot classes from base classes/clutter. 
    \item However, now we see a slight increase as we increase $K$.
    \item The overall few-shot scores increase, which makes sense since the model only has to focus on the few-shot classes (and not having to also distinguish between base classes).

\end{itemize}

\subsection{Visual explanations}
\label{subsec:localisation}


Where does \model\xspace look in an image when given an audio query?
To answer this question, we show Grad-CAM \cite{selvaraju_gradcam_2020} saliency maps for the top five retrieved images based on audio queries for each of the five concepts, see Figure~\ref{tab:qualitative-results}.
Grad-CAM is an explainability method that highlights which parts of the last convolutional layer (and thus the input image) are responsible for producing the predicted similarity score.

These vizualisations are useful for performing implicit localisation of the spoken concepts in the input images, but, perhaps more importantly, they allow us to better understand the model.
Concretely, we observe that
(i) for "broccoli" the model selects the green food in an image;
(ii) "fire hydrant" queries are associated with urban scenes (streets) and tall vertical objects (hydrant, pole, bus);
(iii) the keyword "kite" is linked to people on fields.

While all these associations are useful proxies for identifying the spoken keywords,
they also indicate that the model tends to learn correlations with the context or other spurious features.
This effect is not surprising given that the model learns
in a weakly-supervised manner (the training is done on full images with no explicit localisation information) and
with noisy data (the mined samples are not always accurate, see Figure~\ref{fig:mining-precision-images}).

Note that while the \model\xspace model pools the image features using an attention layer,
the attention weights cannot be used for localisation because the (convolutional) features on which they are applied are further embeded using two linear layers.
These layers mix the spatial information available in the convolutional features and render the attention weights unusable for localisation.
However, we did experiment with a variant of the architecture without the linear image embedding layer and found very similar results in both performance and localisation (using the attention weights) to those obtained with the main model.


\subsection{Removing weak-supervision on image-side}
\begin{table}[h]
	\caption{The few-shot classification scores from \model\ with sampling and no negative base images using a pretrained AlexNet vs.\ a randomly initialised AlexNet.}
	\vspace{-5pt}
	\label{tab:no_pretraining}
	\centering
	\footnotesize
	\renewcommand{\arraystretch}{1.2}	
	\begin{tabular}{ ccccc}
		\toprule
		& & & \multicolumn{2}{c}{Few-shot accuracy}\\
		$K$ & $L_{\mathcal{S}}$ & $L_{\mathcal{M}}$ & With pretrained AlexNet. & Randomly initialised. \\
		\midrule
		5 & 5 & 5 & 89.9 & 90.7\\
		10 & 5 & 5 & 92.0 &91.6 \\
		50 & 5 & 5 & 96.1 & 96.7\\
		100 & 5 & 5 & 95.8 & 95.7\\
		\bottomrule
	\end{tabular}
\end{table}
\begin{itemize}
    \item However, retrieval scores are still lowish. Even for naive approach it stays lowish. What else can be a contributing factor? Maybe the first few layers we use from the pretrained AlexNet?
    \item Improves scores for $K \le$  50 marginally.
    
\end{itemize}

\subsection{Using Insights from Analyses}
\begin{table}[h]
	\caption{}
	\vspace{-5pt}
	\label{tab:improved}
	\centering
	\footnotesize
	\renewcommand{\arraystretch}{1.2}	
	\begin{tabular}{ cccc}
			\toprule
			\multicolumn{1}{c}{$K$}&
			\multicolumn{1}{c}{$L_{\mathcal{S}}$}&
			\multicolumn{1}{c}{$L_{\mathcal{M}}$}&
			\multicolumn{1}{c}{Few-shot accuracy}\\
			\midrule
                5 & 5 & 5 & 89.3\\
			5 & 40 & 5 & \\
			\bottomrule
		\end{tabular}
\end{table}
\begin{itemize}
    \item Since our goal is task, we conclude that for fewer shots mined pairs, removing the base image negatives and the linear image layers helps. We also use no pretrained AlexNet layers in order for us to move to pure few-shot learning on image-side as well.
    
\end{itemize}


==> results.tex <==
\section{Experimental results}

\begin{table}[tb]
	\caption{%
		$P@N$ few-shot retrieval scores (\%) on the five few-shot classes. $K$ is the number of support-set examples per class.	}
	\vspace{-5pt}
	\label{tab:previous_work}
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0.25em}
	\renewcommand{\arraystretch}{1.2}
	\begin{tabular}{ lcccc }
		\toprule
		\multicolumn{1}{c}{Model} & 
		\multicolumn{4}{c}{$K$}\\
		\cline{2-5}
		 & 5 & 10 & 50 & 100 \\
		\midrule
		Naive fine-tuned~\cite{miller_t_exploring_2022} & -- & -- & -- & \textbf{52.5}\\
		Oracle masking~\cite{miller_t_exploring_2022} & -- & 8.4$\pm$0.0  & 24.0$\pm$0.1 & 35.5$\pm$0.2\\
		\smallmodel\ & \textbf{44.3$\pm$0.1} & \textbf{43.4$\pm$0.1} & \textbf{40.4$\pm$0.1} & 42.5$\pm$0.3\\
		\bottomrule
	\end{tabular}
\end{table}

We first want to compare our work directly to that of~\cite{miller_t_exploring_2022}. Concretely, we compare to two of \cite{miller_t_exploring_2022}'s models on the few-shot retrieval task.
The first model we compare to is their naive model, which is trained on background classes and fine-tuned on $K=100$ examples for each of the $L=5$ classes.
The second is their oracle masking model in which the contrastive loss used during fine-tuning %
ensures that a negative image does not contain any instance of the anchor few-shot class.
The results are given in Table~\ref{tab:previous_work} \changed{(where scores are absent, \cite{miller_t_exploring_2022} did not report the scores)}.

Comparing our full \model\ model to the oracle masking approach, we see that we outperform  \cite{miller_t_exploring_2022} consistently across all values of $K$. 
Neither \model\ or oracle masking works as well as the naive fine-tuned approach (line 1), but fine-tuning only works with a large number of shots.
We also see that our approach (a bit surprisingly) delivers approximately the same few-shot retrieval scores as $K$ increases, whereas \cite{miller_t_exploring_2022}'s scores in line~2, increase.
\changed{We investigate the reasons for this in Section~\ref{subsec:retrieval_plateau}.}
Our approach therefore works particularly well with fewer shots.

\begin{table}[tb]
	\caption{%
		Few-shot word classification accuracy scores (\%).
		We vary the number of shots per class $K$. 
		Instead of only considering the five classes from~\cite{miller_t_exploring_2022}, we also look at settings with 40 classes in the support and/or matching sets.}
	\vspace{-5pt}
	\label{tab:few-shot}
	\centering
	\footnotesize
	\renewcommand{\arraystretch}{1.2}	
	\begin{tabular}{cccccc}
		\toprule
		\multicolumn{1}{c}{Model}&
		\multicolumn{1}{c}{$K$}&
		\multicolumn{1}{c}{$L_{\mathcal{S}}$}&
		\multicolumn{1}{c}{$L_{\mathcal{M}}$}&
		\multicolumn{1}{c}{Few-shot accuracy}\\
		\midrule
		\multirow{4}{2cm}{\centering\smallmodel} & 5 & 5 & 5 & 65.4\\
		& 10 & 5 & 5 & 77.5\\
		& 50 & 5 & 5 & 86.6\\
		& 100 & 5 & 5 & \textbf{90.9}\\
		\bottomrule
	\end{tabular}
\end{table}

To work towards a few-shot model in an actual low-resource setting, we now consider our model on the conventional few-shot word classification task (\S\ref{sec:task}). 
This task wasn't used in~\cite{miller_t_exploring_2022}.
Table~\ref*{tab:few-shot} shows that the few-shot classification scores increase as $K$ increases when we use mined pairs.

All together, our results sets a competitive multimodal baseline for both few-shot retrieval and few-shot word classification in settings where the number of shots is small.
\changed{However, before we can consider this model in an actual few-shot setting, we have to analyse the in more depth.}


==> setup.tex <==
\newpage~\newpage~\newpage
\section{Experimental setup}
\label{sec:setup}

\textbf{Data:} 
For our experiments, we use the SpokenCOCO Corpus~\cite{hsu_text-free_2021} which  consists of the MSCOCO~\cite{lin_microsoft_2014} images with recorded spoken captions corresponding to the MSCOCO textual captions.
We %
parametrise the utterances %
as mel-spectograms with a hop length of 10~ms, a window %
of 25~ms and 40~mel bins. %
These are truncated or zero-padded to 1024 frames. 
Images are resized to 224$\times$224 pixels and normalised with means and variances calculated on ImageNet~\cite{deng_imagenet_2009} with VGG~\cite{simonyan_very_2015}.

We use the SpokenCOCO setup of \cite{miller_t_exploring_2022}
by splitting it into two main sets: a set which contains only the few-shot classes and a set that does not contain any of the few-shot classes. %
We refer to the latter set as background data. %
For the set containing the few-shot classes, we further split it into the same training and testing sets as \cite{miller_t_exploring_2022}.
We sample the support set $\mathcal{S}$ from this training set (\S\ref{sec:task}) and use the Montreal forced aligner~\cite{mcauliffe_montreal_2017} to isolate the few-shot words.
For our mining approach (\S\ref{subsec:mining}), we need unlabelled audio and image data to mine pairs from; for this we use the remainder of the training data that does not include the support set.
From these unlabelled collections, we mine pairs: the $n=600$ highest ranking examples per class %
(\S\ref{subsec:mining}).
These pairs are split into training and validation %
pairs.

\textbf{Models:} Figure~\ref{fig:model} illustrates our model, \model\ 
(\S\ref{subsec:model}).
For the image branch, we use an adaption of AlexNet~\cite{krizhevsky_imagenet_2017} to get a sequence of per pixel embeddings. %
We use an adaption of \cite{nortje_towards_2022}'s audio network for the audio branch.
The model is initialised by pretraining it on the background data using the contrastive retrieval loss of \cite{harwath_unsupervised_2016}.
We take $N_\textrm{pos}=5$ and $N_\textrm{neg}=11$ in Equation~\ref{eq:loss} after fine-tuning it on the development pairs.
For validation, we use the development set to get one positive image $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^+$ and one negative image $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^-$ for each developmental word-image $(\boldsymbol{\mathrm{x}}_{\textrm{audio}},\, \boldsymbol{\mathrm{x}}_{\textrm{vision}})$ pair. 
The validation task measures whether the model will place $\boldsymbol{\mathrm{x}}_{\textrm{vision}}$ and  $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^+$ closer to  $\boldsymbol{\mathrm{x}}_{\textrm{audio}}$ than it would to  $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^-$. 
We train all models with Adam~\cite{kingma_adam_2015} for 100 epochs using the validation task for early stopping and a batch size of 8. 
Source code will be released upon acceptance.

\textbf{Few-shot tasks:} Using the same five classes -- \textit{broccoli}, \textit{zebra}, \textit{fire hydrant}, \textit{sheep} and \textit{kite} -- as \cite{miller_t_exploring_2022}, we evaluate our approach on two tasks (as explained in \S\ref{sec:task}): a traditional few-shot classification task and a few-shot retrieval task.
For both these tasks, the $K$-shot $L$-way support set $\mathcal{S}$ contains $K$ ground truth spoken word-image pairs for each of the $L=5$ classes and is used to mine pairs for training and development.
For testing the few-shot classification task, we sample $1000$ episodes where each episode contains $L$ spoken word queries $\boldsymbol{\mathrm{x}}^q_{\textrm{audio}}$, one for each class, and a matching set $\mathcal{M}$ which contains one image $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^{(i)}$ for each class.   
However, in the few-shot retrieval task, instead of having one image per class, $\mathcal{M}$ consists of $5000$ images $\boldsymbol{\mathrm{x}}_{\textrm{vision}}^{(i)}$ where some depicts a few-shot class and others do not. 
Here, 20 query words are taken per class and averaged to get $\boldsymbol{\mathrm{x}}^q_{\textrm{audio}}$. 
For each of the $L$ queries $\boldsymbol{\mathrm{x}}^q_{\textrm{audio}}$, these $5000$ images are ranked from highest to lowest similarity.
The precision at $N$ ($P@N$) score is the proportion of images in the top $N$ highest ranking images that are from the same class as $\boldsymbol{\mathrm{x}}^q_{\textrm{audio}}$.
$N$ is the actual number of images in $\mathcal{M}$ that depicts the word class. 


